Spoofing-Resilient LiDAR-GPS Factor Graph Localization with Chimera Authentication

Many vehicle platforms typically use sensors such as LiDAR or camera for locally-referenced navigation with GPS for globally-referenced navigation. However, due to the unencrypted nature of GPS signals, all civilian users are vulner-able to spoofing attacks, where a malicious spoofer broadcasts fabricated signals and causes the user to track a false position fix. To protect against such GPS spoofing attacks, Chips-Message Robust Authentication (Chimera) has been developed and will be tested on the Navigation Technology Satellite 3 (NTS-3) satellite being launched later this year. However, Chimera authentication is not continuously available and may not provide sufficient protection for vehicles which rely on more frequent GPS measurements. In this paper, we propose a factor graph-based state estimation framework which integrates LiDAR and GPS while simultaneously detecting and mitigating spoofing attacks experienced between consecutive Chimera authentications. Our proposed framework combines GPS pseudorange measurements with LiDAR odometry to provide a robust navigation solution. A chi-squared detector, based on pseudorange residuals, is used to detect and mitigate any potential GPS spoofing attacks. We evaluate our method using real-world LiDAR data from the KITTI dataset and simulated GPS measurements, both nominal and with spoofing. Across multiple trajectories and Monte Carlo runs, our method consistently achieves position errors under 5 m during nominal conditions, and successfully bounds positioning error to within odometry drift levels during spoofed conditions.

==> sections/outline.tex <==
\section*{Outline}
\begin{outline}[enumerate]

\1 Abstract
\1 Introduction
    \2 Precise and robust localization is critical to the operation of autonomous vehicles, as the rest of the autonomy stack depends on its output
    \2 Sensor fusion is state-of-the-art in terms of localization for autonomous vehicles
    \2 A natural pairing is LiDAR with GPS: complementary advantages
    \2 However, GPS is vulnerable to spoofing
        \3 Chimera provides authentication, but not fast enough
    \2 Need to design spoofing resilient sensor fusion
\1 Related Work
    \2 LiDAR-GPS sensor fusion
        \3 Filtering \cite{wan2018robust} \cite{li2021gil}
            \4 \cite{li2021gil} - 
        \3 Graph \cite{he2022lidar} \cite{chen2019probabilistic}
            \4 \cite{he2022lidar} - Uses IMU, 
        \3 Graphs vs. Filtering
            \4 FGO demonstrated superior to EKF \cite{wen2021factor}
            \4 Enable loop closure, updating previous portions of trajectory to better improve current estimates
    \2 Factor graph GPS/Robust FGO 
        \3 \cite{wen2021factor} \cite{wen2021integrity}
    \2 LiDAR-GPS spoofing vulnerability
        \3 \cite{shen2020drift}
    \2 Spoofing-resilient GPS sensor fusion
        \3 \cite{mina2022gps}
        \3 \cite{kanhere2022factor}
\1 Problem Statement
\1 Approach
    \2 Factor graph
        \3 Nodes and edges
            \4 Figure: Graph structure
        \3 Sliding window
    \2 Spoofing detection 
        \3 Test statistic computation
    \2 Spoofing mitigation
        \3 
\1 Results
    \2 Lidar-GPS FGO nonspoofed
    \2 Lidar-GPS FGO spoofed (no spoofing D/M)
    \2 Lidar-GPS FGO spoofed (with spoofing D/M)
    \2 Lidar-GPS FGO spoofed (with spoofing D/M and Chimera)
    \2 Varying environments/trajectories (Lidar uncertainties)
    \2 Varying spoofing attacks
\1 Conclusion

        
        
\end{outline}



